Modelling and Verifying the AODV Routing Protocol

This paper presents a formal specification of the Ad hoc On-Demand Distance Vector (AODV) routing protocol using AWN (Algebra for Wireless Networks), a recent process algebra which has been tailored for the modelling of Mobile Ad Hoc Networks and Wireless Mesh Network protocols. Our formalisation models the exact details of the core functionality of AODV, such as route discovery, route maintenance and error handling. We demonstrate how AWN can be used to reason about critical protocol properties by providing detailed proofs of loop freedom and route correctness.

==> fig/ex_aodv_1.tex <==
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(1.0,0.0){0.2}{d}
   \rput(1.0,0.0){$d$}

   \cnode(0.0,-1.0){0.2}{b}
   \rput(0.0,-1.0){$b$}

   \cnode(-1.0,0.0){0.2}{s}
   \rput(-1.0,0.0){$s$}

   \cnode(0.0,1.0){0.2}{a}
   \rput(0.0,1.0){$a$}


%%  EDGES  %%
   \ncline{s}{a}
   \ncline{a}{b}
   \ncline{b}{d}
   \ncline{s}{b}
   \ncline{a}{d}

\endpspicture


==> fig/ex_aodv_2.tex <==
\pspicture(-10,-10)(10,10)

%%  NODES  %%
\rput(0,0){\textcolor{white}{RREQ}}
\rput(0,0){\textcolor{white}{RREQ}}
\rput(0,0){\textcolor{white}{RREQ}}

   \cnode(1.0,0.0){0.2}{d}
   \rput(1.0,0.0){$d$}

   \cnode(0.0,-1.0){0.2}{b}
   \rput(0.0,-1.0){$b$}

   \cnode(-1.0,0.0){0.2}{s}
   \rput(-1.0,0.0){$s$}

  \cnode(0.0,1.0){0.2}{a}
   \rput(0.0,1.0){$a$}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=1pt]{->}{s}{a}
   \aput[0pt]{:U}{\tiny RREQ~}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=1pt]{->}{a}{s}
   \aput[0pt]{:D}{\tiny ~RREQ}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=1pt]{<-}{b}{s}
   \aput[0pt]{:D}{\tiny RREQ~}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=1pt]{<-}{s}{b}
   \aput[0pt]{:U}{\tiny ~RREQ}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt]{->}{a}{d}
   \aput[0pt]{:U}{\tiny RREQ\ }
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt]{<-}{d}{b}
   \aput[0pt]{:D}{\tiny RREQ\ }
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=1pt]{->}{a}{b}
   \aput[0pt]{:D}{\tiny RREQ\ }
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=1pt]{->}{b}{a}
   \aput[0pt]{:U}{\tiny RREQ\ }

\endpspicture


==> fig/ex_aodv_3.tex <==
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(1.0,0.0){0.2}{d}
   \rput(1.0,0.0){$d$}

   \cnode(0.0,-1.0){0.2}{b}
   \rput(0.0,-1.0){$b$}

   \cnode(-1.0,0.0){0.2}{s}
   \rput(-1.0,0.0){$s$}

   \cnode(0.0,1.0){0.2}{a}
   \rput(0.0,1.0){$a$}

%%  EDGES  %%
   \ncline{a}{b}
   \ncline{b}{d}
   \ncline{s}{b}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt]{<-}{a}{d}
   \aput[0pt]{:U}{\tiny \ RREP}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt]{<-}{s}{a}
   \aput[0pt]{:U}{\tiny \ RREP}

\endpspicture

